The Morbid Realities of Social Media: An Investigation into the Misinformation Shared by the Deceased Victims of COVID-19

Social media platforms have had considerable impact on the real world especially during the Covid-19 pandemic. Misinformation related to Covid-19 might have caused significant impact on the population specifically due to its association with dangerous beliefs such as anti-vaccination and Covid denial. In this work, we study a unique dataset of Facebook posts by users who shared and believed in Covid-19 misinformation before succumbing to Covid-19 often resulting in death. We aim to characterize the dominant themes and sources present in the victim's posts along with identifying the role of the platform in handling deadly narratives. Our analysis reveals the overwhelming politicization of Covid-19 through the prevalence of anti-government themes propagated by right-wing political and media ecosystem. Furthermore, we highlight the failures of Facebook's implementation and completeness of soft moderation actions intended to warn users of misinformation. Results from this study bring insights into the responsibility of political elites in shaping public discourse and the platform's role in dampening the reach of harmful misinformation.

==> Makefile <==
# Makefile for LaTeX files

# Original Makefile from http://www.math.psu.edu/elkin/math/497a/Makefile

# Please check http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile
# for new versions.

# Copyright (c) 2005,2006 (in order of appearance):
#	Matti Airas <Matti.Airas@hut.fi>
# 	Rainer Jung
#	Antoine Chambert-Loir
#	Timo Kiravuo

# Permission is hereby granted, free of charge, to any person obtaining
# a copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to
# permit persons to whom the Software is furnished to do so, subject to
# the following conditions: 

# The above copyright notice and this permission notice shall be
# included in all copies or substantial portions of the Software. 

# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND,
# EXPRESS OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT.
# IN NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY
# CLAIM, DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT,
# TORT OR OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE
# SOFTWARE OR THE USE OR OTHER DEALINGS IN THE SOFTWARE. 

# $Id: Makefile,v 1.18 2006-06-19 10:58:11 mairas Exp $

LATEX	= pdflatex
BIBTEX	= bibtex
MAKEINDEX = makeindex
XDVI	= xdvi -gamma 4
DVIPS	= dvips
DVIPDF  = dvipdft
L2H	= latex2html
GH	= gv

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"

DATE=$(shell date +%Y-%m-%d)

COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi 
RM = rm -f
OUTDATED = echo "EPS-file is out-of-date!" && false

# These are OK

SRC	:= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
TRG	= $(SRC:%.tex=%.dvi)
PSF	= $(SRC:%.tex=%.ps)
PDF	= $(SRC:%.tex=%.pdf)

# These are not

#BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))
#DEP     := $(shell perl -ne '($$_)=/^[^%]*\\include\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $(SRC))
#EPSPICS := $(shell perl -ne '@foo=/^[^%]*\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $(SRC) $(DEP))


define run-latex
	$(COPY);$(LATEX) $<
	egrep $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) >/dev/null; true
	egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	$(RM) $(<:%.tex=%.toc.bak)
	# Display relevant warnings
	egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef

define run-pdflatex
	LATEX=pdflatex
	@$(run-latex)
endef

define get_dependencies
	deps=`perl -ne '($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $<`
endef

define getbibs
	bibs=`perl -ne '($$_)=/^[^%]*\\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $< $$deps`
endef

define geteps
	epses=`perl -ne '@foo=/^[^%]*\\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $< $$deps`
endef

define manconf
	mandeps=`if test -r $(basename $@).cnf ; then cat $(basename $@).cnf |tr -d '\n\r' ; fi`
endef

all 	: $(TRG)

.PHONY	: all show clean ps pdf showps veryclean

clean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.dvi=%.aux) $(TRG:%.dvi=%.bbl) $(TRG:%.dvi=%.blg) $(TRG:%.dvi=%.log) $(TRG:%.dvi=%.out) $(TRG:%.dvi=%.idx) $(TRG:%.dvi=%.ilg) $(TRG:%.dvi=%.ind) $(TRG:%.dvi=%.toc) $(TRG:%.dvi=%.d)

veryclean	: clean
	  -rm -f *.log *.aux *.dvi *.bbl *.blg *.ilg *.toc *.lof *.lot *.idx *.ind *.ps  *~

# This is a rule to generate a file of prerequisites for a given .tex file
%.d	: %.tex
	$(get_dependencies) ; echo $$deps ; \
	$(getbibs) ; echo $$bibs ; \
	$(manconf) ; echo  $$mandeps  ;\
	echo "$*.dvi $@ : $< $$deps $$bibs $$epses $$mandeps" > $@ 

include $(SRC:.tex=.d)

# $(DEP) $(EPSPICS) $(BIBFILE)
$(TRG)	: %.dvi : %.tex
	  @$(run-latex)

$(PSF)	: %.ps : %.dvi
	  @$(DVIPS) $< -o $@

#$(PDF)  : %.pdf : %.dvi
#	  @$(DVIPDF) -o $@ $<
# To use pdflatex, comment the two lines above and uncomment the lines below
#$(PDF) : %.pdf : %.tex
#	@$(run-pdflatex)


show	: $(TRG)
	  @for i in $(TRG) ; do $(XDVI) $$i & done

showps	: $(PSF)
	  @for i in $(PSF) ; do $(GH) $$i & done

ps	: $(PSF) 

pdf	: $(PDF) 

# TODO: This probably needs fixing
html	: @$(DEP) $(EPSPICS)
	  @$(L2H) $(SRC)



######################################################################
# Define rules for EPS source files.

# These rules probably just cause unnecessary confusion, so commenting
# them away for the time being. -- mairas 2005-01-12

#%.eps: %.sxd
#	$(OUTDATED)
#%.eps: %.sda
#	$(OUTDATED)
#%.eps: %.png
#	$(OUTDATED)
#%.eps: %.sxc
#	$(OUTDATED)
#%.eps: %.xcf
#	$(OUTDATED)
#%.eps: %.zargo
#	$(OUTDATED)
#%.eps: %.m
#	@egrep -q $(MPRINT) $< && ($(OUTDATED))


==> tex-files/introduction-old.tex <==
\section{Introduction}
In early 2020, the WHO declared abundance of information
surrounding COVID-19 from a variety of sources as infodemic. An infodemic is
defined as excessive false or misleading information that can cause confusion
and risk-taking behaviors that can harm health.

\para{COVID-19 \& Misinformation}
The 2016 election highlighted the ability of misinformation to influence user
beliefs, behaviors and actions. In recent years, due to increased polarity,
accessibility and information overload, the role of misinformation in the
beliefs of the population has only become more visible. Conspiracy theories such
as QAnon, the alternative facts of the far-right wing and more recently
anti-science beliefs COVID-19, all based on misinformation campaigns have had
seismic consequences on the society.
%
The US alone has lost 94,640 unvaccinated patients to COVID-19, although
COVID-19 has been gradually ascending to the ranks of being a preventable
disease through social guidelines and advancements in vaccinations, the vaccine
hesitancy and covid denial perpetuated by misinformation campaigns have made
advancements to contain COVID-19 in vain. While there are valid medical reasons
to not be vaccinated, the majority of the unvaccinated individuals have their
actions based on their anti-vaccinations beliefs. These anti-vaccination and
anti-masks beliefs are primarily based on misinformation that have been spread
across the US. Similar to the Covid-19, the misinformation surrounding it has
mutated into a contagion of its own, infected through fear, anger and distrust.
%
Victim of the misinformation campaigns propagated online by internet charlatans,
political celebrities and media personalities for their own gains more often
than not suffer great losses in their health.

\para{Herman Cain Award}
The Washington Post noted "the Internet has been a graveyard of stories about
unvaccinated deaths". With the majority of deaths associated with Covid being
that of the unvaccinated population, the demise of anti-vaccination and
anti-mask advocates is no rare occurrence.
%
A series of shared and re-shared misinformation posts and memes conforming to
the anti-vaccine beliefs only to be followed by the eulogies of relatives paint
a macabre picture on the Facebook walls of covid deniers and antivaxxers.
%
Herman Cain, a prominent political figure and an advocate of anti-mask mandates
died at the age of 74 after contracting covid. He became one of the first
examples of advocates of anti-science, anti-mask, and anti-vaccine contracting
Covid-19 soon after his public declaration of anti-mask beliefs.
%
Following his death, crowd sourced collections of cases of people publicly
declaring their anti-mask/anti-vaccine beliefs prior to their hospitalization or
death sprung up to catalog perpetrators, but more often, the victims of
misinformation. The curators of these collections create cases by collecting
memes and misinformation shared by the victims declaring their anti-vaxx or
anti-mask beliefs followed by a post declaring the hospitalization of the
victims and then often a eulogy by a relative.
%
While primarily being a source of schadenfreude and occasionally serving to warn
the audience of the dangers of misinformation, most importantly, the cases call
attention to our collective failure of being unable to prevent preventable
deaths.  By being unvaccinated and not adhering to the social guidelines the
users are on some level direct victims of misinformation propagated by some bad
actors on a platform ignorant or disinterested towards its role in the
ecosystem.
% Do we talk about the significance of the misinformation found here?
\note{This dataset of curated case studies of victims of COVID-19 enables us to
understand how these users adopted beliefs that were harmful to their health.
By looking at what narratives were driving these beliefs, what were the sources
involved in these narratives and the platforms reactions to these harmful
narratives we can better understand the case studies curated in this dataset,}


\para{COVID-19 Narratives}
Politicizing narratives? Conspiratorial Narratives?

\para{Sources}

\note{
\para{Reasons for misinformation}
Research into adoption of misinformation and conspiracy theories suggest
the sources of misinformation and the platform which facilitate its spread
being critical contributors to the propagation and consequent adoption of
misinformation. Pew Research Center noted Americans who relied on information
from either Trump or their personal/community connections were the least likely
to get vaccinated \cite{pewTrump}.
%
Based on these results and prior work on adoption of conspiracy theories, we
focus on the 1) the prominent disseminators of information and 2) the
interventions by the platform in understanding the spread and growth of covid-19
false narratives. We collect the cases of users who publicly advocated coivd
misinformation and were hospitalized after contracting covid. Our goal is to
explore these cases to identify the repeating narratives and prominent
individuals responsible for facilitating the misinformation. Furthermore, we
explore the efforts taken by social media platforms, especially Facebook to flag
dangerous posts and memes.
}

\para{Sources of information}
Fueled by the growing partisanship, the information related to covid-19, its
vaccinations and guidelines have been greatly politicized by few bad actors such
media personalities, politicians, and influencers for their own gains. So much
so, that issue of how to address the outbreak has been the most divisive issue
in the recent years \cite{pewSocialMedia}.
%
Conspiracy theories linking microchips and vaccines, speculating
the governmental origins of the virus, and uncovering hidden covid-19 remedies
have bred distrust in scientific organizations and has manufactured an
atmosphere of doubt and hesitancy towards vaccines which resulted in the deaths
of the victims of such theories and misinformation.
%
In attempts to benefit from the situation, politicians and influences, after
recognizing their disaffected audience, often signaled their support to the
conspiracies casting doubt on the threat of covid and the effectiveness of
countermeasures \cite{chillizza_2022}.
%
In recent years, especially following the Capitol riots, the seismic effects of
misinformation has been made exceedingly evident.
%
In this light, given the case studies of the victims of misinformation and later
covid-19, we seek to identify the sources or the prominent middle men that
repeatedly appear in multiple cases. By identifying prominent individuals and
parties we identify the narratives supported or spread by them.  We hypothesize
many misinformation narratives exploit the users trust in a few
prominent figures for legitimacy.

\para{Responsibility of platforms}
The 2016 elections highlighted the role of social media platforms played in
disseminating misinformation at an alarming rate. Research has repeatedly
demonstrated how social media platforms are exploited to spread propaganda and
misinformation.
%
In addition to being exploited by bad actors, research has also shown the
algorithms, design and structure of social media platforms actively facilitate
the spread of misinformation by disproportionately promoting fake and inciting
news. Studies show, falsehood diffusing significantly further and faster than truth in all
categories of information. This corroborates with the cases  against
Facebook highlighted by the whistle-blower Frances Haugen which outlines
Facebook's algorithms being modeled to maximize engagement which is
inadvertently done by propagating conforming, negative, hateful and incendiary
content.
%
Although many platforms, including Facebook, have made policies and promises to
attempt to eradicate or intervene in fake news and dangerous misinformation its
completeness and effectiveness is yet to be measured independently.
%
With over half of the Americans follow social media for news related to COVID-19
despite the rising criticism of algorithms and the design of platforms in spreading
misinformation and facilitating propaganda along with distrust in the governance
and moderation abilities of the platform, in our work we seek to observe the
misinformation narratives being spread on Facebook.
%
By exploring the cases of Facebook users becoming the victims of misinformation
and then COVID-19, we explore the misinformation narratives still present on
Facebook and identify the failures of Facebook in identifying and intervening in
the spread of misinformation.

\para{Our Contributions}
In this paper, we explore the landscape of misinformation related to COVID-19,
its flow, and its governance found amongst the victims of COVID-19 and
misinformation. We do so by performing quantitative and longitudinal analysis on
the curated anti-vaxxer, anti-mask and covid-hoax posts of victims of COVID-19.
Furthermore, we identify and categorize the sources of misinformation along with
the attempts of platforms, especially Facebook, in blocking these pathways. More
specifically, we seek to explore the following perspectives.


\begin{itemize}
	\item \emph{The COVID-19 narratives}
	\item \emph{The sources of information}
	\item \emph{The intervention strategies of platforms}
\end{itemize}

